Hierarchical Autoscaling for Large Language Model Serving with Chiron

Large language model (LLM) serving is becoming an increasingly important workload for cloud providers. Based on performance SLO requirements, LLM inference requests can be divided into (a) interactive requests that have tight SLOs in the order of seconds, and (b) batch requests that have relaxed SLO in the order of minutes to hours. These SLOs can degrade based on the arrival rates, multiplexing, and configuration parameters, thus necessitating the use of resource autoscaling on serving instances and their batch sizes. However, previous autoscalers for LLM serving do not consider request SLOs leading to unnecessary scaling and resource under-utilization. To address these limitations, we introduce Chiron, an autoscaler that uses the idea of hierarchical backpressure estimated using queue size, utilization, and SLOs. Our experiments show that Chiron achieves up to 90% higher SLO attainment and improves GPU efficiency by up to 70% compared to existing solutions.

==> 0000-intro_v3.tex <==
\section{Introduction}
\label{s:introduction}

% Why is queueing a problem? current queues cannot handle it, why use LSOs with queues? why merge LSOs with queuing


\begin{figure}[!tb]
    \centering
    \includegraphics[width=\linewidth]{resources/QLM_motivation.pdf}
    \caption{Scenarios for workload consolidation in LLM serving systems.}
    \label{fig:scenarios}
\end{figure}


\BLUE{\noindent \textbf{Motivation.} 
The emergence of large language models (LLMs) such as OpenAI GPT-4 and Google Gemini has enabled a wide range of novel AI applications~\cite{compound-ai-blog,bommasani2021opportunities,wu2023autogen}, including chatbots and coding assistants.
Consequently, serving LLMs has become an increasingly critical workload, catering to both enterprise and consumer applications with service-level objectives (SLOs)~\cite{jyothi2016morpheus,qiu2020firm,wang2024efficient}.

Recent work on LLM serving has primarily focused on interactive services, which have strict SLO requirements for inter-token latency and time-to-first token.
In production systems, in addition to these interactive services, there is also a growing need to support batch LLM queries, which are required for tasks such as data wrangling, log processing, and model fine-tuning.
These batch LLM queries have much higher SLO values, ranging from minutes to hours, as they do not require immediate execution.
There is an opportunity for workload consolidation by jointly serving batch and interactive requests to maximize device utilization and reduce the total resource requirement.

Specifically, we identify the following workload consolidation scenarios as shown in Figure~\ref{fig:scenarios}:
\begin{enumerate}[wide=0pt, label=(\alph*)]
    \item \emph{Batch and Interactive Request Co-location}: Instead of using separate LLM serving instances for batch and interactive requests, they can be co-located on a single LLM serving instance.
    A major challenge that arises with such co-location is that interactive requests may need to wait at the front of the waiting queue before execution on the LLM serving instance, causing head-of-line (HOL) blocking. To prevent such HOL blocking, an alternative strategy is to evict existing batch requests from the LLM serving instance and put them back into the waiting queue. This effectively allows interactive requests to be executed immediately in a nearly isolated manner. 
    Compared to traditional DNN serving systems, request eviction in LLM serving requires saving the state, i.e. the KV cache or output tokens to minimize throughput disruption for the batch requests.
    
    \item \emph{Multi-model Batch Request Co-location:} Instead of using multiple LLM serving instances for each model, the same serving instance could be used with the models being swapped in and out on demand. However, as LLMs are much larger compared to DNN models, the swap times are also much larger ( for e.g. $\sim$20s for a 70B parameter model).
    Consequently, serving requests in their order of arrival for multiple models can lead to repeated model swapping and loss in throughput.
    Instead, \emph{requests groups} can be created per model, and this grouping reduces required model swaps and minimize loss in throughput. 
\end{enumerate}

Both of these scenarios require the management of a \emph{global request queue} that comprise a mix of interactive and batch requests with multiple models.
Previous work on LLM serving~\cite{kwon2023efficient,yu2022orca,tensorrt,tgi,aiops2024qiu,li2023alpaserve,sheng2023flexgen,wu2023fast} has largely focused on interactive requests where maintaining global queues is unnecessary, as it would lead to violation of strict request latency requirements.
For example, Lluminix~\cite{llumnix} autoscales and adds new LLM serving instances when the queue size exceeds a threshold.
However, when the workload comprises of a combination of batch and interactive requests, maintaining request queues can be beneficial as it presents opportunities for resource savings while still adhering to latency requirements, as discussed in the two scenarios above.

% \begin{figure}[t]
%     \hspace{-3ex}
%     \centering
%     \begin{minipage}{.1\textwidth}
%         \centering
%         \includegraphics{resources/results/Intro_diagram_HOL_blocking.pdf}
%         \label{fig:Predictable Waiting Time}
%     \end{minipage}%
%     \hspace{11ex}
%     $\vpointer$
%     \centering
%     \begin{minipage}{.2\textwidth}
%     \centering
%     \includegraphics{resources/results/Intro_diagram_latency.pdf}
%     \label{fig:swaping_with_reordering}
%     \end{minipage}%
%     \hfill
%     \vspace{-20pt}
%     \caption{\sysname nearly eliminates HOL blocking time in both single and multi-model serving scenarios and enables SLO attainment for batch and latency-sensitive applications. }
%     \label{fig:intro_result}
% \end{figure}

% -> why waiting time???
% However, serving LLMs can be surprisingly resource-intensive and costly.
% For example, a single A100 GPU is only able to serve $<$1 request per second for a medium-sized model with 13 billion parameters.
% State-of-the-art LLM serving systems such as vLLM~\cite{kwon2023efficient}, Orca~\cite{yu2022orca}, and TensorRT-LLM~\cite{tensorrt} improve serving throughput by upto 20$\times$ over traditional ML serving systems with novel techniques such as \emph{continuous batching}~\cite{yu2022orca} and \emph{paged attention}~\cite{kwon2023efficient}.
% (e.g., with \textit{continuous batching}~\cite{yu2022orca} and \textit{PagedAttention}~\cite{kwon2023efficient})


%LLM serving systems have HOL blocking problem,
%QLM introduces LSOs and optimizes them for 
\noindent
\textbf{Our Contributions.}
% Achieving end-to-end latency SLOs together with throughput and utilization goals is challenging.
% To address this problem, we introduce \sysname, a queue management framework for SLO-oriented LLM serving.
We present \sysname, a system for workload consolidation in LLM serving that manages the global request queue to minimize the total resource usage while maximizing SLO satisfaction.
\sysname leverages three major ideas in its queue management framework:
\begin{enumerate}[wide=4pt,label=(\alph*)]
\item \emph{Request Group Abstraction:}
\sysname uses \emph{request groups}, where requests that share the same performance characteristics (i.e. model and latency SLO) are grouped together and decisions are taken per request group instead of per request.
Decision making at the per-request group level offers two advantages: 
\begin{enumerate*}
    \item Request groups are a natural abstraction for scenarios such as multi-model swapping (shown in Scenario 1), and
    \item Requests groups improve system scalability by reducing the overhead of decision making. 
\end{enumerate*}
\sysname places these request groups in virtual queues that determine the order in which requests are consumed by the LLM serving instances.

\item \emph{Request Waiting Time (RWT) Estimator:}
When making decisions on order in requests groups, it is beneficial to estimate queue waiting time to ensure that SLOs are met.
However, estimating the waiting time is challenging because the execution time for a request depends on its output token length, which is unknown apriori before executing the request~\cite{kwon2023efficient} (i.e., stochastic in nature).
We observe and mathematically prove that despite these stochastic effects, the waiting time in LLM serving is predictable and provide an estimator for it.

\item \emph{Global Scheduler:}
Finally, \sysname uses a \emph{Global Scheduler} (described in Section~\ref{s:plan_generation}) that leverages the waiting time estimates of request groups to create an optimal ordering and assignment of request groups onto the virtual queues to maximize SLO attainment.
\end{enumerate}


\noindent \textbf{Results.}
We demonstrate \sysname on vLLM~\cite{kwon2023efficient} as the backend LLM-serving system.
\sysname uses the following four basic LLM Serving Operations (LSOs) to manage the request queue (see \cref{s:lso} for details):
\begin{enumerate*}[label=(\arabic*)]
\item \emph{Request Pulling} from the global waiting queue into the running batch in the GPU,
\item \emph{Request Eviction} from the running batch back into the waiting queue,
\item \emph{Model Swapping} from CPU to GPU memory, and
\item \emph{Load Balancing} across multiple LLM model instances.
\end{enumerate*}

We evaluate \sysname on three popular LLMs of varying sizes (i.e., Mistral-7B~\cite{mistral}, Vicuna-13B~\cite{vicuna}, and Llama-70B~\cite{touvron2023llama}) on heterogeneous GPU clusters with NVIDIA A10 and A100 GPUs.
We adopt workloads from a real-world LLM dataset: ShareGPT~\cite{shareGPT} using setups derived from our production requirements.
Our experiments demonstrate the following major improvements with \sysname:
\begin{enumerate}[wide=0pt,label=(\arabic*)]
    \item \emph{SLO Attainment:} \sysname achieves 40--90\% higher SLO attainment compared to the vanilla vLLM serving system and 50--90\% higher SLO attainment compared to traditional ML serving systems like SHEPHERD,
    \item \emph{Request Throughput:} \sysname improves the request throughput in a multi-model serving system by 400\% on average and in a single-model serving system by 20\% on average compared to other LLM serving systems, and
    \item \emph{LSO Ablation Study:} \sysname demonstrates that all LSOs contribute to SLO attainment and throughput improvement.
    Notably, we find that model warm start improves throughput by 300\% in multi-model serving, and request eviction improves SLO attainment by 80\% in single-model serving.
\end{enumerate}
}
% \noindent
% \textbf{Putting \sysname in Perspective.}
% In production LLM serving, it is critical to support effective multi-model queue management and scale to a large number of LLMs~\cite{hu2021lora,sheng2023slora} with varying SLO requirements and request rates while ensuring high throughput and device utilization.
% % \hq{Effective queue management is the key to multi-model LLM serving, which often confronts the significant challenge of device shortage and queue accumulation but device under-utilization, from our experience as a major cloud provider offering ML-as-a-Service.}
% \sysname is the first queue management framework that enforces the end-to-end latency SLOs while improving LLM-serving throughput and device utilization by systematically orchestrating backend LSOs.
% % (1) existing LLM serving frameworks that ignore SLOs are already covered in the intro
% % (2) existing SLO-aware model serving frameworks
% Previous frameworks do not apply to LLMs because the per-request execution time is variable and nondeterministic, which, combined with continuous batching behavior, affects the decision-making for each LSO.
% Andes~\cite{liu2024andes} defines Quality-of-Experience (QoE) for LLM serving as token delivery speed and proposes a preemptive scheduler that maximizes QoE.
% However, Andes does not enforce the end-to-end latency SLO, only optimizes for one LSO (e.g., request preemption), and negatively impacts system throughput by up to 10\%.




% 1. Reordering of queue based on a queue abstraction …..
%     1. Some of these are distributions …. Based on Bayes estimator (how is profiling done for these? Using this data, which is to minimize uncertainty and determine distribution of key parameters, how are these parameters decided you can talk later)
% 2. If there are distributions, then each is modeled with a This paper investigates SLO and LSO based-modeling because in the end SLO is the decided parameter that the customer demand, and no method uses it as the central parameter of optimization, while there are SLO-based parameters for model serving they lack this

% Our model serving is based on addressing 3 key challenges: 1. How best to optimize the queue? (a) continuous reprioirtizng queue entries to achieve what? Optimal queue length for the highest priority job.. there are uncertainty in the model serving parameters that can be handled with bayesian stats using profiling data for such and such… 3. using stochastic programming,2.  bayesian model gives you the distribution for chosen parameters: waiting time and completion time main uncertainties based on profiling data from 


% The major parameter of the queue total completion time and waiting time, these are stochastic they are not deterministic and we determine these disitrbutions with profiling to build a Bayesian model to determine the best estimates for these two distributions. And our results are so much better…. Doesnt take into account uncertainty, no reordering, 


% SLOs are the prime metric and no one uses these in the most effective way and purpose of this paper as an SLO-driven model parameters, put those results at the beginning, even though there are other SLO-based approaches we are better because….. 1. 2. 3.  That are indeed the inadequacies of the previous work….. handling uncertainty and no way… they do normal optimization which as we show is insufficient, to achieve….


% Make connection of the previous work….. here are the issues of the previous work…. You dont have to say this is how we address it…. 


% By not doing dynamic reordering they are stuck 

% Role of the SLO in deciding priority per-user, in the process we see significant uncertainty is in the wait time and overall execution time, we go to the data

% Contributions of this work are:

% While determining this SLO, now with the SLO these SLOs can be highly variable and introduce, now we have uncertainty under control we can use stochastic programming,


% Need to determine key parameters because you have talked about queue parameters previously - mean based analysis how much worse can you get?

%separate paragraph: service is not quantized, dont assume 
%explanation of cascading effect
%promotes continual chance that request will meet its SLO, second benefit is that service times are stochastic, benefit of being stochastic previous people assume it to be constant which is based on a few samples, mean value approach doesnt take into account variance of the distribution and the only way to do that is to get full posterior using Bayesian
%now that you have distribution you use a stochastic solver (give detailed results)
%you can maintain higher throughput but you will be missing many SLO deadlines, need to make distributon of service times (whatever the metric is)

==> 0002-design.tex <==
\section{\sysname Design Overview}
\label{s:design}

\begin{figure}[!b]
    \centering
    \includegraphics{resources/Teleios.pdf}
    \caption{Overview of \sysname.}
    \label{fig:qlm_overview}
\end{figure}

\sysname aims to maximize latency SLO satisfaction in LLM serving workloads.
To do so, \sysname manages a global request queue and orchestrates multiple LLM Serving Operations (LSOs) to reorder and drain the global queue.


\subsection{Lifecycle of a Request in \sysname}
To explain the design of \sysname (as shown in Figure~\ref{fig:qlm_overview}), we first walk through the lifecycle of a request generated from applications to completion.
LLM-augmented applications generate requests that are received at the \sysname API gateway.
These requests are added to a global queue where they wait until being served.
To prevent the global queue from being a single point of failure, it is implemented with a distributed message broker such as RabbitMQ~\cite{rabbitmq} that provides the requisite fault tolerance and consistency properties.

% lifecycle step 1
\noindent
\textbf{Formation of Request Groups.}
Every incoming request is grouped with other requests that share common performance characteristics (such as model type, SLO value, and token distribution) to form \textit{Request Groups}.
This converts the complexity of the optimization problem from per-request level to per-request-group level.
By doing so, it alleviates the scalability challenges and lowers optimization overheads.
Additionally, request groups are a useful abstraction in the multi-model serving case as described in Section~\ref{ss:characterization}. 
Request grouping criteria and details are described in \cref{s:virtual_queues}.

% \noindent \textbf{Request Groups to Reduce Overhead.}
% As actions for multiple backend LSOs are set when serving requests from the global queue, \sysname needs to solve a multi-dimensional optimization problem that involves SLOs, model type, waiting time, etc.
% Solving such an optimization problem per-request is not scalable due to the high solving overhead.
% Hence, to reduce such overhead, \sysname uses the notion of \emph{request groups} that scales down the input space for the optimization problem.
% \sysname creates these request groups based on the performance demand/requirement characteristics of requests.
% We identify input/output tokens, SLOs, and model types as the necessary features to capture the entire performance spectrum.

% lifecycle step 2
\noindent
\textbf{Assigning Request Groups to Virtual Queues.}
Requests in a request group are then assigned to a \textit{Virtual Queue}, representing a waiting queue for an LLM serving instance in the cluster.
The introduction of virtual queues creates a common abstraction for setting the actions of backend LLM Serving Operations (LSOs) such as request pulling, request eviction, load balancing, and model swapping.
The ordering of the request groups in a virtual queue determines the execution ordering of the requests on the corresponding LLM serving instance.
We refer readers to \cref{s:virtual_queues} for virtual queue formation and \cref{s:lso} for the translation from virtual queue ordering to LSO actions.


% \noindent \textbf{Virtual Queues as an LSO Abstraction.}
% Additionally, we introduce the notion of \emph{virtual queues} that creates a common abstraction for setting the actions of underlying LSOs.
% A \emph{virtual queue} is an ordering of request groups that are served by an LLM serving instance.
% Multiple virtual queues are used by \sysname, and each virtual queue corresponds to its own LLM serving instance.
% The virtual queue ordering sets LSO actions using \sysname agents resident on each LLM serving instance.
% For example, to configure the request eviction LSO, changes in the head of the virtual queue are monitored by a \sysname agent.

% lifecycle step 3
\noindent
\textbf{Virtual Queue Reordering for SLO Attainment Maximization.}
While requests are assigned to request groups in a first-come-first-serve manner, request groups in a virtual queue are reordered to maximize the SLO attainment for all requests being served.
At the core of SLO attainment maximization are \sysname's \emph{request waiting time (RWT) estimator} (see \cref{s:base_estimator}) and \emph{global scheduler} (see \cref{s:plan_generation}).

% \noindent \textbf{RWT Estimator and global scheduler for SLO Translation.}
% \sysname's translation of SLOs to virtual queue ordering and consequently LSO actions is enabled by the \emph{request waiting time (RWT) estimator} and \emph{global scheduler}.
% The RWT estimator calculates completion times from the virtual queue and the global scheduler uses these estimates to reorder the virtual queues and satisfy SLOs.
% The \textit{RWT estimator} (described in Section~\ref{s:base_estimator}) estimates the time required to serve this newly added request based on its position in the virtual queue.
% If the estimation is higher than the actual SLO value, then an SLO violation is detected and the \textit{global scheduler} is invoked to re-order all the virtual queues in an attempt to satisfy the SLO value.
% The global scheduler does this reordering based on a stochastic programming solver (described in Section~\ref{s:plan_generation}).

\noindent
\textbf{Request Execution.}
Each request, when being moved to the head of the virtual queue, will be executed on the LLM serving instance, and the output will be returned to the application.
This completes the lifecycle of a request.

We illustrate the rationale of \sysname's design choices and workflow in the next section (\cref{ss:design-principles}).

\subsection{\sysname Design Principles}
\label{ss:design-principles}

We highlight the major design principles underpinning \sysname, derived from large-scale production LLM serving workload requirements at a major cloud provider.

\noindent \textbf{Design Principle \#1: \textit{Scaling to a high request arrival rate and burstiness.}}
\sysname must be able to handle a high volume of requests for SLO attainment without the overhead that compromises the serving throughput.
Existing model-serving frameworks that leverage optimization techniques such as linear programming have exponential or cubical complexity, which limits the scalability to larger workloads and longer queues.
\sysname instead introduces \textit{request groups} to reduce the input space of the optimization solvers, thus lowering the computational overhead and enabling scalability.

\noindent
\textbf{Design Principle \#2: \textit{Handling multiple LSOs with inter dependencies.}}
To attain model-serving latency SLOs, it is critical to translate the latency SLO to the appropriate backend LSO actions.
\sysname models these complex inter-relationships with a two-step approach.
First, \textit{virtual queues} enable the necessary abstraction to enable actions for multiple backend LSOs.
Second, the \textit{global scheduler} models the impact of ordering on multiple LSOs with a linear programming solver. 
\BLUE{We specifically prefer a linear programming solver over other optimization methods because it systematically considers various constraints introduced by multiple LSOs, SLO constraints, and waiting time estimates from the RWT estimator.
}

\noindent
\textbf{Design Principle \#3: \textit{Handling heterogeneous models and hardware device configurations.}}
LLM serving workloads consist of diverse model types with vastly different computational requirements, SLOs, and token length distributions.
Hardware device configurations are also heterogeneous in terms of computing power, GPU memory capacity, and GPU-CPU memory bandwidth.
To efficiently map LLM requests to the appropriate hardware resources, \sysname's global scheduler has to consider each device's computing power, memory capacity, and memory bandwidth.
The \textit{RWT estimator} estimates this impact of heterogeneity for the global scheduler.
The profiling costs for the RWT estimator are minimal, only a single batch run for a given combination of request group and GPU device is needed.
Hence, \sysname does not require significant training when adding new LLM models or GPU devices into the serving cluster.

==> 0007-discussion.tex <==
\section{Discussion and Future Work}
\label{s:discussion}

\noindent \textbf{What happens if \sysname is unable to meet SLOs?}
%business question
\sysname's global scheduler may not be able to find an optimal virtual queue ordering if the request demand is high and the number of LLM serving instances (i.e., underlying compute resources) is insufficient.
In such cases, we have three choices:
\begin{enumerate*}[label=(\alph*)]
    \item scale up the number of LLM serving instances by adding GPU devices, as we demonstrate in Figure~\ref{fig:multi_model_slos} and Figure~\ref{fig:single_model_SLOs}, 
    \item fall back to a heuristic such as Earliest Deadline First (EDF) and continue serving requests, and
    \item performance admission control or rate limiting by dropping incoming requests to limit queue size.
\end{enumerate*}
Option (a) can only be used when there are available resources, whereas Option (b) and Option (c) would lead to SLO violations.

\noindent \textbf{Can new LSOs be added to \sysname?}
\sysname can be extended to support other LSOs that depend on the queue size and request ordering.
For example, GPU partitioning techniques (such as NVIDIA MIG~\cite{mig}) can be added as an LSO with additional constraints on memory in the linear programming solver described in \cref{s:plan_generation}.
We leave the addition of extra LSOs to our future work.

\noindent \textbf{How can \sysname handle request priorities?}
\sysname can also be used when strict priorities are assigned to requests instead of SLO values.
In the strict priority model, $request_1$ would execute before $request_2$, if $priority(request_1)$ < $priority(request_2)$.
With strict priority, the relative ordering of requests across priorities is pre-decided, however per-priority assignment still needs to be optimized to maximize SLO satisfaction.
Consequently, the concepts of virtual queues, request groups, and the RWT estimator continue to remain useful. 

\noindent \textbf{Can SLOs be defined on end-to-end latency?}
\BLUE{\sysname addresses the problem of optimizing time to first token (TTFT) SLO attainment.
However, it can also be made to work with the modified objective of end to end request completion time SLOs (i.e. including decoding iterations).
In this case, the RWT estimator and global scheduler need to be modified to consider a distribution of number of output tokens per request (as the exact number are unknown aprioiri).}

\noindent \textbf{Can SLOs be defined on inter-token latency?}
\sysname primarily addresses the problem of TTFT and does not guarantee the inter-token latency (ITL).
However, related work such as Andes~\cite{liu2024andes} attempts to guarantee token generation speed (that can be converted into inter-token latency) by modifying the local vLLM scheduler.
\sysname can work together with such systems to ensure ITL SLOs along with TTFT SLOs.





%per/GPU throughput graphs for TTFT, ITL, both
% -- assume 3x spikes for interactive (x instances for interactive, 2x for mixed, y batch)
%SLO (time to convergence is high for Lluminix)
% --- varying arrival rates for batch and interactive
%hysteresis associated with autoscaling // non-critical
%RWT estimator(done)

%Lluminix batch size of 4


%Vary arrival rates for interactive requests
% TTFT SLO
% QLM :  
% Lluminix :

% ITL SLO
% QLM:  
% Lluminix: 

%Varying arrivals for batch requests
%TTFT SLO
% QLM: 
% LLuminix: 

%Vary arrival rates for interactive requests
% Avg throughput per instance
% QLM :  
% Lluminix :

%Vary arrival rates for batch requests
% Avg throughput per instance
% QLM :  
% Lluminix :

%Batch size variation with different models

%Queue size vs SLO

%RWT estimator


